Scalable HPC and AI Infrastructure for COVID-19 Therapeutics

COVID-19 has claimed more 1 million lives and resulted in over 40 million infections. There is an urgent need to identify drugs that can inhibit SARS-CoV-2. In response, the DOE recently established the Medical Therapeutics project as part of the National Virtual Biotechnology Laboratory, and tasked it with creating the computational infrastructure and methods necessary to advance therapeutics development. We discuss innovations in computational infrastructure and methods that are accelerating and advancing drug design. Specifically, we describe several methods that integrate artificial intelligence and simulation-based approaches, and the design of computational infrastructure to support these methods at scale. We discuss their implementation and characterize their performance, and highlight science advances that these capabilities have enabled.

==> innovation.tex <==
We (hope to) investigate 100B drug candidates. Although still small relative
to the full chemical space of possibilities, it is still (among) the largest,
if not the largest chemical space sampled.

There are three main contributing factors to the unprecedented number of drug
candidates “sampled”: 

\begin{enumerate}
\item  Multiple levels of algorithmic innovation (e.g.,
DeepDriveMD)
\item Improvements arising from “AI driven MD”, as well as “MD
driven AI” (!)
\item Each stage in IMPECCABLE is effective stand-alone, when coupled together
the collective effectiveness is greater. Performance improvement as a
consequence of AI-driven MD and MD-driven AI.

\item  Advanced tools to support multiple heterogeneous
workflows at scale. 

\end{enumerate}

Ultimately, (i) and (ii) yield: reduced “flops per effective drug candidate”
screened, without increasing false positive or false negative ratios. (iv)
results in a high-peak and sustained flop count, as well as throughput (=
number of drug candidates screened per unit physical time).


==> misc.tex <==
\section{Introduction}
ACM's consolidated article template, introduced in 2017, provides a
consistent \LaTeX\ style for use across ACM publications, and
incorporates accessibility and metadata-extraction functionality
necessary for future Digital Library endeavors. Numerous ACM and
SIG-specific \LaTeX\ templates have been examined, and their unique
features incorporated into this single new template.

If you are new to publishing with ACM, this document is a valuable
guide to the process of preparing your work for publication. If you
have published with ACM before, this document provides insight and
instruction into more recent changes to the article template.

The ``\verb|acmart|'' document class can be used to prepare articles
for any ACM publication --- conference or journal, and for any stage
of publication, from review to final ``camera-ready'' copy, to the
author's own version, with {\itshape very} few changes to the source.

\section{Template Overview}
As noted in the introduction, the ``\verb|acmart|'' document class can
be used to prepare many different kinds of documentation --- a
double-blind initial submission of a full-length technical paper, a
two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
journal article, a SIGCHI Extended Abstract, and more --- all by
selecting the appropriate {\itshape template style} and {\itshape
  template parameters}.

This document will explain the major features of the document
class. For further information, the {\itshape \LaTeX\ User's Guide} is
available from
\url{https://www.acm.org/publications/proceedings-template}.

\subsection{Template Styles}

The primary parameter given to the ``\verb|acmart|'' document class is
the {\itshape template style} which corresponds to the kind of publication
or SIG publishing the work. This parameter is enclosed in square
brackets and is a part of the {\verb|documentclass|} command:
\begin{verbatim}
  \documentclass[STYLE]{acmart}
\end{verbatim}

Journals use one of three template styles. All but three ACM journals
use the {\verb|acmsmall|} template style:
\begin{itemize}
\item {\verb|acmsmall|}: The default journal template style.
\item {\verb|acmlarge|}: Used by JOCCH and TAP.
\item {\verb|acmtog|}: Used by TOG.
\end{itemize}

The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
\begin{itemize}
\item {\verb|acmconf|}: The default proceedings template style.
\item{\verb|sigchi|}: Used for SIGCHI conference articles.
\item{\verb|sigchi-a|}: Used for SIGCHI ``Extended Abstract'' articles.
\item{\verb|sigplan|}: Used for SIGPLAN conference articles.
\end{itemize}

\subsection{Template Parameters}

In addition to specifying the {\itshape template style} to be used in
formatting your work, there are a number of {\itshape template parameters}
which modify some part of the applied template style. A complete list
of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

Frequently-used parameters, or combinations of parameters, include:
\begin{itemize}
\item {\verb|anonymous,review|}: Suitable for a ``double-blind''
  conference submission. Anonymizes the work and includes line
  numbers. Use with the \verb|\acmSubmissionID| command to print the
  submission's unique ID on each page of the work.
\item{\verb|authorversion|}: Produces a version of the work suitable
  for posting by the author.
\item{\verb|screen|}: Produces colored hyperlinks.
\end{itemize}

This document uses the following string as the first command in the
source file:
\begin{verbatim}
\documentclass[sigconf,authordraft]{acmart}
\end{verbatim}

\section{Modifications}

Modifying the template --- including but not limited to: adjusting
margins, typeface sizes, line spacing, paragraph and list definitions,
and the use of the \verb|\vspace| command to manually adjust the
vertical spacing between elements of your work --- is not allowed.

{\bfseries Your document will be returned to you for revision if
  modifications are discovered.}

\section{Typefaces}

The ``\verb|acmart|'' document class requires the use of the
``Libertine'' typeface family. Your \TeX\ installation should include
this set of packages. Please do not substitute other typefaces. The
``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
as they will override the built-in typeface families.

\section{Title Information}

The title of your work should use capital letters appropriately -
\url{https://capitalizemytitle.com/} has useful rules for
capitalization. Use the {\verb|title|} command to define the title of
your work. If your work has a subtitle, define it with the
{\verb|subtitle|} command.  Do not insert line breaks in your title.

If your title is lengthy, you must define a short version to be used
in the page headers, to prevent overlapping text. The \verb|title|
command has a ``short title'' parameter:
\begin{verbatim}
  \title[short title]{full title}
\end{verbatim}

\section{Authors and Affiliations}

Each author must be defined separately for accurate metadata
identification. Multiple authors may share one affiliation. Authors'
names should not be abbreviated; use full first names wherever
possible. Include authors' e-mail addresses whenever possible.

Grouping authors' names or e-mail addresses, or providing an ``e-mail
alias,'' as shown below, is not acceptable:
\begin{verbatim}
  \author{Brooke Aster, David Mehldau}
  \email{dave,judy,steve@university.edu}
  \email{firstname.lastname@phillips.org}
\end{verbatim}

The \verb|authornote| and \verb|authornotemark| commands allow a note
to apply to multiple authors --- for example, if the first two authors
of an article contributed equally to the work.

If your author list is lengthy, you must define a shortened version of
the list of authors to be used in the page headers, to prevent
overlapping text. The following command should be placed just after
the last \verb|\author{}| definition:
\begin{verbatim}
  \renewcommand{\shortauthors}{McCartney, et al.}
\end{verbatim}
Omitting this command will force the use of a concatenated list of all
of the authors' names, which may result in overlapping text in the
page headers.

The article template's documentation, available at
\url{https://www.acm.org/publications/proceedings-template}, has a
complete explanation of these commands and tips for their effective
use.

\section{Rights Information}

Authors of any work published by ACM will need to complete a rights
form. Depending on the kind of work, and the rights management choice
made by the author, this may be copyright transfer, permission,
license, or an OA (open access) agreement.

Regardless of the rights management choice, the author will receive a
copy of the completed rights form once it has been submitted. This
form contains \LaTeX\ commands that must be copied into the source
document. When the document source is compiled, these commands and
their parameters add formatted text to several areas of the final
document:
\begin{itemize}
\item the ``ACM Reference Format'' text on the first page.
\item the ``rights management'' text on the first page.
\item the conference information in the page header(s).
\end{itemize}

Rights information is unique to the work; if you are preparing several
works for an event, make sure to use the correct set of commands with
each of the works.

\section{CCS Concepts and User-Defined Keywords}

Two elements of the ``acmart'' document class provide powerful
taxonomic tools for you to help readers find your work in an online
search.

The ACM Computing Classification System ---
\url{https://www.acm.org/publications/class-2012} --- is a set of
classifiers and concepts that describe the computing
discipline. Authors can select entries from this classification
system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
commands to be included in the \LaTeX\ source.

User-defined keywords are a comma-separated list of words and phrases
of the authors' choosing, providing a more flexible way of describing
the research being presented.

CCS concepts and user-defined keywords are required for all short- and
full-length articles, and optional for two-page abstracts.

\section{Sectioning Commands}

Your work should use standard \LaTeX\ sectioning commands:
\verb|section|, \verb|subsection|, \verb|subsubsection|, and
\verb|paragraph|. They should be numbered; do not remove the numbering
from the commands.

Simulating a sectioning command by setting the first word or words of
a paragraph in boldface or italicized text is {\bfseries not allowed.}

\section{Tables}

The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
high-quality tables.

Table captions are placed {\itshape above} the table.

Because tables cannot be split across pages, the best placement for
them is typically the top of the page nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and the
table caption.  The contents of the table itself must go in the
\textbf{tabular} environment, to be aligned properly in rows and
columns, with the desired horizontal and vertical rules.  Again,
detailed instructions on \textbf{tabular} material are found in the
\textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more
desirable. Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

\section{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of the three are
discussed in the next sections.

\subsection{Inline (In-text) Equations}
A formula that appears in the running text is called an inline or
in-text formula.  It is produced by the \textbf{math} environment,
which can be invoked with the usual
\texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
and structures, from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
examples of in-text equations in context. Notice how this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols and
structures available in \LaTeX\@; this section will just give a couple
of examples of display equations in context.  First, consider the
equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\section{Figures}

The ``\verb|figure|'' environment should be used for figures. One or
more images can be placed within a figure. If your figure contains
third-party material, you must clearly identify it as such, as shown
in the example below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{The 1907 Franklin Model D roadster.}
\end{figure}

Your figures should contain a caption which describes the figure to
the reader. Figure captions go below the figure. Your figures should
{\bfseries also} include a description suitable for screen readers, to
assist the visually-challenged to better understand your work.

Figure captions are placed {\itshape below} the figure.

\subsection{The ``Teaser Figure''}

A ``teaser figure'' is an image, or set of images in one figure, that
are placed after all author and affiliation information, and before
the body of the article, spanning the page. If you wish to have such a
figure in your article, place the command immediately before the
\verb|\maketitle| command:
\begin{verbatim}
  \begin{teaserfigure}
    \includegraphics[width=\textwidth]{sampleteaser}
    \caption{figure caption}
    \Description{figure description}
  \end{teaserfigure}
\end{verbatim}

\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, an article in a proceedings (of a conference,
  symposium, workshop for example) (paginated proceedings article)
  \cite{Andler79}, a proceedings article with all possible elements
  \cite{Smith10}, an example of an enumerated proceedings article
  \cite{VanGundy07}, an informally published work \cite{Harel78}, a
  doctoral dissertation \cite{Clarkson85}, a master's thesis:
  \cite{anisi03}, an online document / world wide web resource
  \cite{Thornburg01, Ablamowicz07, Poker06}, a video game (Case 1)
  \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05} and
  (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, sections are lettered, not
numbered. This document has two appendices, demonstrating the section
and subsection identification method.

\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{itemize}
\item {\verb|sidebar|}:  Place formatted text in the margin.
\item {\verb|marginfigure|}: Place a figure in the margin.
\item {\verb|margintable|}: Place a table in the margin.
\end{itemize}

==> overview.tex <==



==> performance.sj.tex <==
%!TEX root = main.tex

\subsection{WF1: Ensemble Consensus Docking}\label{ssection:expwf1}

Compared to physics-based simulation methods, docking is a relatively
inexpensive computational process. To increase the reliability of docking
results, multiple docking protocols for the same ligand set and protease are
preferred over individual docking scores. WF1 uses OpenEye and Autodock-GPU.
The former is executed on x86 architectures (e.g., Frontera); the latter on
GPUs (e.g., Summit).

For each of the identified receptor sites, WF1 iterates through a list of
ligands and computes a docking score for that ligand-receptor pair. The score
is written to disk and is used as filter to identify ligands with favorable
docking results (score and pose). The docking call is executed as a Python
function in OpenEye, and as a self-contained task process in AutoDock-GPU. In
both cases, the RAPTOR framework (\S~\ref{sssection:raptor}) is used for
orchestration.

The duration of the docking computation depends on the type of CPU (OpenEye) or
GPU (AutoDock-GPU) used, and the computational requirements of each individual
receptor. We measure the docking time (seconds) and docking rate (docks/hr) of
three use cases: (1) production runs for NVBL-Medical Therapeutics campaigns;
and runs for largest achievable size on (2) Frontera and (3) Summit.
Table~\ref{tab:wf1} summarizes the parameterization and results of the
experiments we performed for each use case.

\begin{table*}
  \centering
  \begin{tabular}{ c  % p{1.6cm}  % Use case  % {\textwidth}
                   l  % p{1.6cm}  % HPC platform
                   l  % p{1.6cm}  % docking software
                   r  % p{1.7cm}  % # compute Nodes
                   r  % p{1.7cm}  % # pilots
                   r  % p{2.1cm}  % # ligands
                   r  % p{2.1cm}  % utilization
                   r  % p{1.2cm}  % min  docking time
                   r  % p{1.8cm}  % max  docking time
                   r  % p{1.5cm}  % mean docking time
                   r  % p{1.5cm}  % min  docking rate
                   r  % p{1.5cm}  % max  docking rate
                   r} % p{2.2cm}  % mean docking rate
  %
  \toprule
  %
  \textbf{Use}                               &
  \multirow{2}{*}{\textbf{Platform}}         &
  \multirow{2}{*}{\textbf{Application}}      &
  \multirow{2}{*}{\textbf{Nodes}}            &
  \multirow{2}{*}{\textbf{Pilots}}           &
  \textbf{Ligands}                           &
  \multirow{2}{*}{\textbf{Utilization}}      &
  \multicolumn{3}{c}{\textbf{Docking Time [sec]}}  &
  \multicolumn{3}{c}{\textbf{Docking Rate [$\times10^6$ docks/hr]}}  \\
  %
  \cline{8-13}
  %
  \textbf{Case} &
                &
                &
                &
                &
  \textbf{[$\times10^6$]}  &
                &
  \textbf{min}  &
  \textbf{max}  &
  \textbf{mean} &
  \textbf{min}  &
  \textbf{max}  &
  \textbf{mean} \\
  %
  \midrule
  %
  1             &  % Use case
  Frontera      &  % HPC platform
  OpenEye       &  % docking software
  128           &  % # compute Nodes
  31            &  % # pilots
  370           &  % # smiles
  89.6\%        &  % # utilization
  0.1           &  % min  docking time
  3582.6        &  % max  docking time
  28.8          &  % mean docking time
  0.2           &  % min  docking rate
  17.4          &  % max  docking rate
  5.0           \\ % mean docking rate
  %
  2             &  % Use case
  Frontera      &  % HPC platform
  OpenEye       &  % docking software
  3850         &  % # compute Nodes
  1             &  % # pilots
  125           &  % # smiles
  95.5\%        &  % # utilization
  0.1           &  % min  docking time
  833.1         &  % max  docking time
  25.1          &  % mean docking time
  16.0          &  % min  docking rate
  27.5          &  % max  docking rate
  19.1          \\ % mean docking rate
  %
  3             &  % Use case
  Summit        &  % HPC platform
  AutoDock-GPU  &  % docking software
  1000         &  % # compute Nodes
  1             &  % # pilots
  57            &  % # smiles
  $\approx$95\% &  % # utilization
  0.1           &  % min  docking time
  263.9         &  % max  docking time
  36.2          &  % mean docking time
  10.9          &  % min  docking rate
  11.3          &  % max  docking rate
  11.1          \\ % mean docking rate
  %
  \bottomrule
  %
  \end{tabular}
  \caption{WF1 use cases. For each use case, RAPTOR uses one pilot for each
  receptor, computing the docking score of a variable number of ligands to that
  receptor. OpenEye and AutoDock-GPU implement different docking algorithms and
  docking scores, resulting in different docking times and rates. However,
  resource utilization is $>=$90\% for all use cases.}
  \label{tab:wf1}
\end{table*}

WF1 assigns one pilot for each receptor for which a set of ligands will be
docked. Within each pilot, one master task is executed for every $\approx$100
nodes. Each master iterates at different offsets through the ligands database,
using pre-computed data offsets for faster access, and generating tasks to be
distributed to the worker tasks. One worker is placed on each compute node,
waiting for the master to send docking requests. Once received, the worker
distributes those requests across the CPU cores, or GPUs for execution.

% For OpenEye, the docking operation is executed as a function call on
% Frontera's CPU cores, while Autodock-GPU is executed as a stand-alone,
% self-contained process (i.e., task) on Summit's GPU. \amnote{we mention
% function call vs. task before already, could be removed.}

% ------------------------
\subsubsection{Use Case 1}

We assign each of the 31 receptors to a single pilot \textemdash{} which are
independent jobs submitted to the batch-queue. Due to the different batch-queue
waiting times, at most 13 concurrent pilots executed concurrently. With 13-way
pilot concurrency, we reached a peak of $\approx17.4\times10^6$ docks/hr but it
should be noted that on Frontera, we were able to use only 34 cores per node out
of the 56 available in order to keep an acceptable load on the shared
filesystem.

Figs.~\ref{sfig:wf1_uc1_durations_short} and~\ref{sfig:wf1_uc1_durations_long}
show the distribution of the docking times for receptors with the shortest and
longest average docking time for a given ligand set. All the other receptors,
have similar long-tailed distributions. Across the 31 receptors, the
min/max/mean docking times are 0.1/3582.6/28.8 seconds (Tab.~\ref{tab:wf1}),
posing a challenge to scalability due to the communication and coordination
overheads. The long tail of the docking times requires load balancing docking
functions across the available workers in order to maximize resource
utilization and minimize overall execution time.

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/oe_frontera_29.times.png}
    \caption{ }
    \label{sfig:wf1_uc1_durations_short}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/oe_frontera_20.times.png}
    \caption{ }
    \label{sfig:wf1_uc1_durations_long}
  \end{subfigure}
  \caption{WF1, Use Case 1: Distribution of docking runtimes for the receptor
    with the (a) shortest and (b) longest average docking time out of the 31
    receptors analyzed. The distributions of all 31 receptors have a long tail.
    \jhanote{The quality of these pictures is insufficient to read axes labels
    or markings. We also need consistency across: Docking hit, Docking call and
    Docking (call) Time.  We say this is a distribution of runtimes, but our
    x-axis is labelled as duration.  }\amnote{pictures will be fixed, we will
    consistently say 'docking time'}\jhanote{I am not able to reproduce 5.0M
    from 28.8}\amnote{Not sure what the 5M reference - was that a previous
    version of plots / text maybe?}}
  \label{fig:wf1_uc1_durations}
\end{figure}

We addressed load balancing in three ways: (i) tasks are communicated in bulk so
as to limit the communication frequency and therefore overhead; (ii) multiple
master processes are used to limit the number of workers served by each master,
avoiding bottlenecks; (iii) multiple concurrent pilots are used to partition the
docking computations of the set of ligands. 

% Fig.~\ref{sfig:wf1_uc1_utilization} shows the percentage of pilot resources
% (i.e., cores) utilized when docking. Overall, core utilization depends on: (i)
% docking time \textemdash{} shorter call durations lead to task rates and
% respective overheads; and (ii) the number of docking calls. The receptors in
% Fig.~\ref{sfig:wf1_uc1_utilization} are ordered by mean docking time, but
% receptors 0 and 29 had only a small number of ligands to analyze, 5\% and 10\%
% of the total set, respectively. For smaller numbers of ligands, the relative
% overheads of initialization and termination become more significant, reducing
% resource utilization.

% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/wf0_utilization.png}
%     \caption{\jhanote{Please make the legend for x and y axis LARGER}}
%     \label{sfig:wf1_uc1_utilization}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/wf1/oe_frontera_p.rates.png}
%     \caption{\jhanote{Use engineering/scientific notation for x-axis so as to prevent bleeding}}
%     \label{sfig:wf1_uc1_througput}
%   \end{subfigure}
%     \caption{WF1, Use Case 1: (a) \% of core utilization \jhanote{Utilization is
%           already expressed as a percentage}\mtnote{I am not sure I understand
%           your comment. Better?} for each of the 31 pilots assigned to a
%           receptor. Receptors are ordered by mean docking time, mean utilization
%           is $89.6\%$.  (b) Cumulative docking rates (across all pilots) as a
%           function of time; throughput varies as the number of active pilots
%           varies with time.}
%   \label{fig:wf1_uc1_durations}
% \end{figure}

Figs.~\ref{sfig:wf1_uc1_rate_short} and~\ref{sfig:wf1_uc1_rate_long} show the
docking rates for the pilots depicted in
Figs.~\ref{sfig:wf1_uc1_durations_short} and~\ref{sfig:wf1_uc1_durations_long}
respectively. As with dock time distributions, the docking rate behavior is
similar across pilots and therefore receptors.  It seems likely that the
repeated increases and decreases of the rate depend on the interplay of
different conditions: machine performance; size of the pilot; and specific
properties of the docked ligands and the target receptor.  We measure a min/max
docking rate of $0.2/17.4\times10^6$ docks/hr with a mean of $5\times10^6$
docks/hr (Tab.~\ref{tab:wf1}). 

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/oe_frontera_29.rates.png}
    \caption{}
    \label{sfig:wf1_uc1_rate_short}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/oe_frontera_20.rates.png}
    \caption{ }
    \label{sfig:wf1_uc1_rate_long}
  \end{subfigure}
  \caption{WF1, Use Case 1: Docking rates for the receptor with  (a) shortest,
           and (b) longest average docking time.}
  \label{fig:wf1_uc1_rate}
\end{figure}

% ------------------------
\subsubsection{Use case 2}
\label{sssec:wf1-uc2}

Fig.~\ref{sfig:wf1_uc1_time_hero} shows the distribution of docking times of
approximately $125\times10^6$ ligands to a single receptor using OpenEye on
Frontera. The distribution has a min/max of 0.1/833.1 seconds and a mean of 25.1
seconds (Tab.~\ref{tab:wf1}).

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1//oe_frontera_h.times.png}
    \caption{ }
    \label{sfig:wf1_uc1_time_hero}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1//oe_frontera_h.rates.png}
    \caption{ }
    \label{sfig:wf1_uc1_rate_hero}
  \end{subfigure}
  \caption{WF1, Use Case 2: (a) Distribution of docking time and (b) docking
           rate for a single receptor and $120\times10^6$ ligands. Executed with
           31 pilots (each using 128 compute nodes/4,352 cores on TACC
           Frontera.}
  \label{fig:wf1_uc1_hero}
\end{figure}

Fig.~\ref{sfig:wf1_uc1_rate_hero} shows the docking rate for a single pilot
with 3850 compute nodes and 130,900 cores. Compared to Use Case 1, the rate
does not present multiple peaks and valleys. After an initial peak at
$\approx27.5\times10^6$ docks/hr, the rate set \jhanote{``rate set on'' does
not read right} on a steady state of $\approx19\times10^6$ docks/hr until the
end of the execution (Tab.~\ref{tab:wf1}). Note that this run was terminated
by Summit's batch system at the end of the given walltime, thus
Fig.~\ref{sfig:wf1_uc1_rate_hero} does not show the ``cool down'' phase.

Use Case 2 reached 95.5\% core utilization, but due to filesystem performance
limitations, we were able to utilize only 34 cores per node, out of the 56
available.

% ------------------------
\subsubsection{Use case 3}
\label{sssec:wf1-uc3}

Figure~\ref{sfig:wf1_uc1_time_summit_hero} shows the distribution of the docking
times of  $\approx57\times10^6$ ligands to a single receptor using AutoDock-GPU
on Summit. The distribution has a min/max of 0.1/263.9 seconds, and a mean of
36.2 seconds. The max docking time is shorter than both Use Case 1,
Fig.~\ref{sfig:wf1_uc1_time_hero} and Use Case 2,
Fig.~\ref{fig:wf1_uc1_durations}, but the mean is longer.

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/ad_summit_h.times.png}
    \caption{ }
    \label{sfig:wf1_uc1_time_summit_hero}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/wf1/ad_summit_h.rates.png}
    \caption{ }
    \label{sfig:wf1_uc1_rate_summit_hero}
  \end{subfigure}
  \caption{WF1, Use Case 3: (a) Distribution of docking time and (b) docking
           rate for a single receptor and $57\times10^6$ ligands. Concurrently
           executed on 6000 GPUs on ORNL Summit.}
  \label{fig:wf1_uc1_summit_hero}
\end{figure}

Fig.~\ref{sfig:wf1_uc1_rate_summit_hero} shows the docking rate for a single
pilot with 1000 compute nodes, i.e., 6000 GPUs. Different from Use Case 1 and 2,
the rate peaks very rapidly at $\approx11\times10^6$ docks/hr and maintains that
steady rate until the end of the execution. Cool down phase is also very rapid.
Also for this use case, we do not have enough data to explain the observed
sustained peak docking rate. As with Use Case 2, we assume an interplay between
the docking implementation in AutoDock-GPU and specific features of the
$57\times10^6$ docked ligands.

Different from OpenEye on Frontera, AutoDock-GPU bundles 16 ligands into one GPU
computation in order to efficiently use the GPU memory, reaching an average
docking rate of $11.1\times10^6$ docks/hr (Tab.~\ref{tab:wf1}). Currently, our
profiling capabilities allow us to measure GPU utilization with 5\% relative
error. Based on our profiling, we utilized between 93 and 98\% of the available
GPU resources.

% In absolute terms, Use Case 2 docking rate is 1.7 times higher, but when
% considering the proportion of CPU cores/GPUs, Use Case 3 has more than twice
% the rate, using 6000 GPUs versus 134,912 CPU cores. \jhanote{I do not
% understand the last sentence}


% ------------------------------------------------------------------------------
\subsection{WF2: ML-driven enhanced Sampling}\label{ssection:expwf2}

<<<<<<< HEAD
WF2 is an iterative pipeline composed of 4 stages. After the first iteration
of the 4 stages is completed, the next iteration starts simulating the
outliers found in the first iteration, or continues the simulations from the
previous iteration if no outliers were found.  The pipeline stops once a
predefined number of iterations have been performed.

We measure RCT overhead and resource utilization through WF2 runs to identify
the performance bottlenecks of the iterative pipeline. We define RCT overhead
as the time spend not executing at least one of the workflow tasks such as RP
bootstrapping environments, EnTK communicating with RabbitMQ (RMQ), and EnTK
and RP to communicate while workloads wait to execute. Resource utilization is
the percentage of time used to execute the given workflow. 
\jhanote{Propose an alternative definition: Resource utilization is the
percentage of time when resources are busy executing tasks. Alternatively, it
is the fraction of utilized nodes to available nodes averaged over the
duration of the workflow.}
=======
WF2 is a an iterative pipeline composed of 4 stages. After the first iteration
of the 4 stages is completed, the new iteration starts simulating the outliers
found in the first iteration or repeating the simulations of the first
iterations if no outliers were found.  The pipeline stops once a predefined
number of iterations have been performed.

We measure RCT overhead and resource utilization through WF2 runs to
identify the performance bottlenecks of the iterative pipeline.
We define RCT overhead as the time spend not executing at least one of the
workflow tasks such as RP bootstrapping environments, EnTK communicating with 
RabbitMQ (RMQ), and EnTK and RP to communicate while workloads wait to execute. 
Resource utilization is the percentage of time spent on computing units i.e. 
CPUs/GPUs for executing a workflow.
>>>>>>> bbca12d67138a4bf2580830a81c9cc084d341b4d

We completed performance evaluation of WF2 to understand existing implementation
and the blue bars in fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} show RCT
overheads for the first version of WF2 (DeepDriveMD v1) and how the RCT overhead
<<<<<<< HEAD
grew with the number of iterations. Depending on the physical system,
DeepDriveMD may require a large number of iteration. Thus, our goal was to both
reduce RCT overhead but, most importantly, to make it invariant of the number of
iterations.

% Based on the analysis of those initial results, domain scientists optimized some
% aspects of WF2, 

An initial analysis suggested multiple optimizations of WF2: some of these
involved improving the deep learning model, algorithms and implementation of
outlier detection, inter alia. These will be reported elsewhere. For the
current investigation, we focused on improving the communication protocol
between EnTK and RMQ, and on reducing the communication latency between EnTK
and RMQ. We avoided sharing connections to RMQ among EnTK threads, reduced the
number of concurrent multiple connections and reused communication channels
whenever possible. Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} (orange)
shows the combined effects of improving DeepDriveMD and EnTK communication
protocol. Overheads were reduced by 57\% compared to
=======
grew with increased iterations. Depending on the physical system, iterations can
grow quickly; thus, our goal was to both reduce RCT overhead but, most 
importantly, to make it invariant with a large number of iterations.

Based on the analysis of those initial results, domain scientists optimized some
aspects of WF2 while we focused on improving the communication protocol between
EnTK and RMQ, and on reducing the communication latency between EnTK and RMQ. We
avoided sharing connections to RMQ among EnTK threads, reduced the number of
concurrent multiple connections and reused communication channels whenever
possible. Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} (orange) shows the
combined effects of improved WF2 and EnTK communication protocol.
Overheads were reduced by 57\% compared to
>>>>>>> bbca12d67138a4bf2580830a81c9cc084d341b4d
Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} (blue) but they were still
growing with the number of iterations.

We moved our RMQ server to Slate, a container orchestration service offered by
OLCF. This dramatically reduced the communication latency between EnTK and
RMQ, as shown in Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} (green).
Thanks to this last improvement, we managed to keep RCT overheads invariant up
to 8 WF2 iterations.

% WF2 is designed to keep track of the progress during multiple iterations and
% maintaining consistent communication is necessary to prevent failures when the
% workflow finished the iterations halfway through.

% profiled RabbitMQ for WF2 runs using the RCT/EnTK debugging mode and made a
% few changes in the communication protocol to address high network latency
% caused by RabbitMQ. The first changed is the application-level optimization.

% minimized connections, reduced message exchange rate. Pika python library for
% RabbitMQ recommends not to share a connection between threads and therefore
% EnTK components open multiple connections for a single run of WF2 but reuse
% channels and connections for message publishing and consuming. We examined the
% control flow of EnTK and removed redundancies, especially to deal with delayed
% messages as the existing implementation uses a continuation-passing style
% asynchronous methods %blockingconnection for the state update.

% Orange color bars in Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh}
% represents this application-level optimization showing 57 percent reduced
% overhead for eight iterations.

% The another change we made is to offer a direct access via Slate.
% ORNL provides Slate, a container orchestration service built by RedHat
% Openshift and Kubernetes, and we use Slate to deploy RabbitMQ on the Marble
% cluster which has InfiniBand connectivity to Summit because we focus on reduced
% latency at a low failure rate on a local network.
% %(fewer routes guarantees less failure)
% For example, single pub/sub message communication requires approximately 15 TCP
% packets and the existing RabbitMQ on TACC Jetstream shows 36.5ms average round
% trip time (RTT) for each packet whereas Slate on the Marble cluster has less
% than 1ms average RTT. Green color bars in
% Fig.~\ref{fig:ml_driven_enhanced_sampling_rct_ovh} show the difference in
% task performance improved significantly while low latencies were provided.

\begin{figure}[h]
  \centering
  %\includegraphics[width=.4\linewidth]{./figures/ai_enhanced_sampling_for_ipdps_graph}
  \includegraphics[width=\linewidth]{figures/wf2_ovh.pdf}
  \caption{RCT overhead reduction with improved WF2, EnTK and RabbitMQ.}
  \label{fig:ml_driven_enhanced_sampling_rct_ovh}
\end{figure}

% \Description{The abstract structure of DeepDriveMD is represented by the
% graph. Stages of the workflow are described as a vertex and the directed edges
% show a sequence of tasks that have different flows to process. Conditional
% workflows have multiple edges as it can have alternative path to proceed.
% Edges can be associated with certain values like data size and elapsed time
% value to calculate total cost/weight/length. }

We found that maximizing resource utilization required data parallelism in
every stage of WF2, but for the MD simulations that were already running
concurrently. Some optimizations out of scope of this investigation, yielded
data parallelism for  data aggregation, ML and outlier detection stages.
Fig.~\ref{fig:wf2-ru} shows resource utilization of WF2, improved
version of EnTK and RMQ on Slate, when executing four pipeline iterations on
Summit, with 20, 40, and 80 compute nodes. Overall, we measured 91\%, 91\%,
89\% utilization respectively. Fig.~\ref{fig:wf2-ru} shows differences in some
of the pipeline stage execution time across scales but, importantly, no
relevant increase of the time spent without executing at least one task.
\jhanote{Although very similar, we should not interchange WF2 and DeepDriveMD.
I replaced DeepDriveMD in the paragraph above with WF2, also to be consistent
with Fig. 9}

%
% Among these,
%
% The data conversion stage uses Python multiprocessing with MPI to take two
% files per rank so that distributed resources are used to aggregate multiple
% trajectory files from MD simulations.
%
% The training stage is optimized with Hyperparameters by EnTK (with a JSON
% file), and the outlier detection stage also runs in parallel for model
% selection and generating embeddings.
%

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/wf2_ru.pdf}
  \caption{WF2 Resource Utilization: 20 nodes (left), 40 nodes (center), and 80
           nodes (right).}
  \label{fig:wf2-ru}
\end{figure}

% \Description{The abstract structure of DeepDriveMD is represented by the
% graph. Stages of the workflow are described as a vertex and the directed edges
% show a sequence of tasks that have different flows to process. Conditional
% workflows have multiple edges as it can have alternative path to proceed.
% Edges can be associated with certain values like data size and elapsed time
% value to calculate total cost/weight/length. }
% \label{fig:ml_driven_enhanced_sampling_distributed}

% TODO: time to completion, along with resource utilization
% TODO: not about pytorch, nvidia version, but horovod

% \begin{figure}[h]
%   \centering
%   %\includegraphics[width=.4\linewidth]{./figures/ai_enhanced_sampling_for_ipdps_graph}
%   \includegraphics[width=.4\linewidth]{figures/streaming_pseudo.png}
%   \caption{Concurrent task execution}
%   %\Description{The abstract structure of DeepDriveMD is represented by the graph. Stages of the workflow are described as a vertex and the directed edges show a sequence of tasks that have different flows to process. Conditional workflows have multiple edges as it can have alternative path to proceed. Edges can be associated with certain values like data size and elapsed time value to calculate total cost/weight/length. }
%     \label{fig:ml_driven_enhanced_sampling_streaming}
% \end{figure}

%The abstract structure of DeepDriveMD is represented by the Fig~\ref{fig:ml_driven_enhanced_sampling} and the integration with other workflows i.e. C1 and ESMACS is visible in the graph. Four stages of the workflow are described as a vertex and the directed edges show a sequence of tasks that have different flows to process. Conditional workflows have multiple edges as it can have alternative path to proceed. For example, $E_1$, $E_2$, and $E_3$ are not traversed if CVAE training is not necessary during the iteration. Edges can be associated with certain values like data size and elapsed time value to calculate total cost/weight/length.

% \subsection{WF3 Execution Performance}

% \jhanote{Describe performance using multi-DVM at 1000 and 2000 nodes
% (Mikhail)}

% We performed initial test runs using the multi-DVM execution mode and observed that executions were stable when each DVM was running on $< 50$ nodes and executing $< 200$ tasks. Beyond that, we observed  interruptions or connectivity losses between executors and bounded DVMs. Further investigation will establish the causes of the observed limits and possible solutions for higher scalability.

% We run \wfcg on 1000 compute nodes (+ 1 node for a RP sub-agent), executing 6000 1-GPU tasks (Fig.~\ref{fig:wf3cg_1000_utilization}) on 32 concurrent DVMs. Each DVM spawned across up to 32 nodes and executed up to 192 tasks. The pilot startup time is longer than when using a single DVM~\cite{summit}, mainly due to the time spent on launching DVMs which, currently, is a sequential process. It took 336 seconds to start 32 DVMs, including 10 seconds sleep time after each DVM startup as an artificial delay implemented in RP to let DVM finalize running operations. Each following task has an extended pre-execution time, which includes time for scheduling and execution preparation (e.g., exec command construction), due to sequential task pre-processing. The process of scheduling differs from non-multi-DVM approach with additional operation of determining DVM id by a node assigned to task. As well as exec command construction process includes 0.1s time delay to let DVM finalize the previous task launching.

% \begin{figure}[h]
%   \begin{center}
%     \includegraphics[width=\linewidth]{figures/wf3cg_1000_utilization.pdf}
%   \end{center}
%   \caption{RCT utilization for \wfcg using multi-DVM}\label{fig:wf3cg_1000_utilization}
% \end{figure}

% We also run \wfcg on 2000 compute nodes (+ 1 node for a RP sub-agent), doubling the number of tasks and DVMs compared to the run with 1000 nodes. At that scale, we observed three main issues: (i) DVM startup failure (1 DVM failed after startup and 1 DVM did not start); (ii) an internal failure of PRRTE (``the topology information for the following node is missing''); and (iii) lost connectivity with the DVMs (``PRUN: DEFHANDLER WITH STATUS LOST\_CONNECTION\_TO\_SERVER(-101)''). The majority of tasks were successfully completed (11802 out of 12000), but those issues prevented RP Task Manager to gracefully handle their termination.

% Concurrent Binding Free Energy

\subsection{Hybrid Workflows using Heterogeneous
Tasks}\label{ssection:expwfhybrid}

%\jhanote{Please use WF3, WF4 and Hybrid here}

WF3 and WF4 are the most computationally intensive methods, costing several
orders of magnitude more node-hours per ligand than
WF1~\cite{saadi2020impeccable}. As discussed in
\S~\ref{ssection:infwfhybrid}, WF3 and WF4 both compute binding free energies,
but have workloads comprised of distinct tasks \textemdash{} GPU-based OpenMM,
and CPU-based NAMD tasks respectively. By merging WF3 and WF4 into a single
hybrid workflow, this provides an opportunity to improve resource utilization
by utilizing RP's unique ability to concurrently execute distinct tasks on CPU
and GPU parts of a node. We evaluate the capability of heterogeneous task
placement using RP in the context of hybrid workflows by examining the
following three performance measures: (i) RCT overheads as a function of
scale; (ii) scalability as a function of problem and resource size, and (iii)
resource utilization.

% with are three-fold: (a) if RCT is lightweight for task-level
% parallelism in hybrid workflows at scale, (b) RCT scalability with regard to
% problem size and resource size, and (c) resource utilization of RCT-enabled
% hybrid workflows.

Figure \ref{fig:overhead_hybrid_base} compares RCT overhead to workflow time
to completion (TTX)  on 32 nodes for different tasks counts, which represent
different production workflow configurations. The TTX in
Fig.~\ref{fig:overhead_hybrid_base}(c) illustrates concurrent execution of GPU
and CPU tasks. The modest increase in TTX compared to
Fig.~\ref{fig:overhead_hybrid_base}(b) is likely due to interference arising
from shared resources across tasks (Fig.~\ref{fig:hybrid}), and some scheduler
inefficiency. A careful evaluation and optimization will form the basis of
further investigation. Fig.~\ref{fig:overhead_hybrid_base}(d) plots the TTX
for the \emph{Hybrid-LB} scenario when the number of WF3 and WF4 tasks are
selected to ensure optimal resource utilization. The number of WF3 in
Fig.~\ref{fig:overhead_hybrid_base}(d) tasks completed is twice the number of
WF3 in Fig.~\ref{fig:overhead_hybrid_base}(c), with no discernible increase in
TTX.

% where
% \emph{ESMACS} denotes OpenMM tasks running on GPU, \emph{TIES} denotes NAMD
% tasks running on CPU, \emph{Hybrid} refers hybrid OpenMM and NAMD tasks with
% heterogeneous task placement, and \emph{Hybrid-LB} refers \emph{Hybrid} with
% load balance to overlap CPU and GPU workload.

% We see that for \emph{ESMACS}, RCT overhead is higher (11.5\%) than others
% due to two reasons: (a) high file staging overhead in I/O (150 ligands to
% process) and (b) comparatively small TTX. Overall, hybrid workflows with
% concurrent OpenMM and NAMD tasks incurs RCT overhead of only 3.8\%
% (\emph{Hybrid}) and 3.9\% (\emph{Hybrid-LB}). The leftmost two panels show
% that TTX of GPU tasks is shorter compared to CPU tasks. For the optimal
% processor utilization discussed in Section 3.4.3, we adjust the TTX of GPU
% tasks to overlap with CPU by processing more ligands on GPU for static load
% balance. As shown in the rightmost two panels, the TTX of \emph{Hybrid-LB}
% remains the same compared to \emph{Hybrid}. Note the fact that both
% \emph{Hybrid} and \emph{Hybrid-LB} TTX are higher than running CPU or GPU
% tasks alone is due to prolonged workflow runtime from sharing public resources
% (e.g., shared host memory access) when running CPU and GPU tasks concurrently.

For configurations of Fig.~\ref{fig:overhead_hybrid_base}(c) and
Fig.~\ref{fig:overhead_hybrid_base}(d), Fig.
\ref{fig:resource_utilization_hybrid_base} depicts resource usage for
different (internal) RCT states as a time-series. ``Green space'' represents
unused resources; ``dark'' represents resource usage. WF3 and WF4 have 4 and 3
stages respectively, which can be discerned from black bars.
Fig.~\ref{fig:resource_utilization_hybrid_base}(b) shows greater ``dark
space'' and thus resource utilization than Fig.
\ref{fig:resource_utilization_hybrid_base}(a), representing greater
computation overlap between GPUs and CPUs due to workload sizing. Both have
higher resource utilization than configurations in
Fig.~\ref{fig:overhead_hybrid_base}(a),(b) due to concurrent CPU and GPU
usage.

%than Fig.\ref{fig:resource_utilization_hybrid_base}(a)


% both between RCT stages (middle blocks) and within an RCT stage (right-most
% blocks). The \emph{Hybrid-LB} configuration in
% Fig.\ref{fig:resource_utilization_hybrid_base}(b) has

% There exist 4 stages of
% computation (4 stages of CPU tasks overlap with 3 stages of GPU tasks) by
% grouping the black bars (\emph{Exec Cmd}).



% which in turn selection overlapping GPU
% computation with CPU as much as possible.

% experimentally
% has better resource utilization than \emph{Hybrid} by overlapping GPU
% computation with CPU as much as possible.



% Compared to
% \emph{Hybrid}, less green bars (\emph{Idle}) are present for \emph{Hyrbid-LB}


\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/overhead_rct_hybrid_base.pdf}
  \end{center}
  \caption{RCT Overhead in Hybrid Workflows.}\label{fig:overhead_hybrid_base}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/resource_utilization_hybrid_base.pdf}
  \end{center}
  \caption{RCT Resource Utilization in Hybrid Workflows.}\label{fig:resource_utilization_hybrid_base}
\end{figure}

Fig.~\ref{fig:overhead_hybrid_scaling} shows the scalability of hybrid
workflows with load balance enabled up to 22,640 tasks on 128 nodes of Summit.
The left two panels demonstrate comparison between 5660 homogeneous tasks (all
GPU tasks) and 5660 heterogeneous tasks (5400 GPU tasks + 260 CPU tasks). An
important observation is that RCT overheads for heterogeneous task placement
is no greater than overheads for homogeneous task placements. RCT overheads
remain essentially invariant with larger workloads with proportionately
increasing node counts (weak scaling).

In Figs.~\ref{fig:overhead_hybrid_base} and \ref{fig:overhead_hybrid_scaling},
RCT overheads vary from 3.8\% to 11.5\% of TTX. The task durations for these
experiments however, are significantly smaller than production task durations,
primarily by reducing the number of timesteps in the MD and equilibrations
stages. The overheads are essentially invariant of task runtimes \textemdash{}
as they arise due to stage transitions and data movement, which are reproduced
with fidelity, thus in production runs, the overheads are significantly less
proportion of TTX.


% We see that employing heterogeneous task placement reduces RCT overhead from
% 8.2\% to 3.9\%, since replacing 260 CPU tasks with 260 GPU tasks increases
% resource requirements of GPU, compared to concurrent CPU and GPU computation.

% For hybrid workflows with heterogeneous tasks, RCT overhead is comparatively
% low in all scenarios (3.9\% for 32 nodes, 4.8\% for 64 nodes, and 5.3\% for
% 128 nodes).

% The reason why RCT overhead is slightly increasing with more ligands on more
% nodes is that RCT need to spend more time to bootstrap and to terminate RCT
% components (e.g., units and pilots) for a larger number of nodes.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/overhead_rct_hybrid_scaling.pdf}
  \end{center}
  \caption{RCT Overhead in Hybrid Workflows at Scale.}\label{fig:overhead_hybrid_scaling}
\end{figure}

Once confirmed the validity of the implemented science, we are now scaling
WF3--4 to a larger number of nodes. Initially, we are focusing on WF3 and, once
achieved the desired scale, we will move on to WF4 and finally to their hybrid
execution. We performed initial test runs using the multi-DVM execution mode
described in \S\ref{sssection:multidvm}, and observed that executions were
stable when each DVM was running on $< 50$ nodes and executing $< 200$ tasks.
Beyond that, we observed  interruptions or connectivity losses between executors
and bounded DVMs. Further investigation will establish the causes of the
observed limits and possible solutions for higher scalability.

We run \wfcg on 1000 compute nodes (+1 node for a RP sub-agent), executing 6000
1-GPU tasks on 32 concurrent DVMs. Each DVM spawned across up to 32 nodes and
executed up to 192 tasks. Fig.~\ref{fig:wf3cg_1000_utilization} shows the
utilization of the available resources across different stages of the execution.
The pilot startup time (blue) is longer than when using a single
DVM~\cite{turilli2019characterizing}, mainly due to the time spent on launching
DVMs which, currently, is a sequential process. It took 336 seconds to start 32
DVMs, including 10 seconds sleep time after each DVM startup as an artificial
delay implemented in RP to let DVM finalize running operations. Each task
requires time to prepare the execution (purple), which mainly includes time for
scheduling the task on a DVM, construct the execution command, and process
placement and launching by the DVM. The scheduling process takes longer than
with a single DVM as it requires to determine which DVM should be used. Further,
the construction of the execution command includes a 0.1s delay to let DVM
finalize the previous task launching. As each operation is done sequentially
per RP executor component, the 0.1s delay accounts for 600s alone.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=\linewidth]{figures/wf3cg_1000_utilization.pdf}
  \end{center}
  \caption{RCT utilization for \wfcg using multi-DVM.}\label{fig:wf3cg_1000_utilization}
\end{figure}

WF3 allows for arbitrarily decide the number of simulation steps. We used
500,000 steps for our test run, 1/10 of the steps required by a production run.
This reduced the walltime required for our test, without affecting our
performance analysis. The time taken by each task to execute does not affect
pilot startup time, execution preparation and pilot termination time. Looking at
Fig.~\ref{fig:wf3cg_1000_utilization}, using 10 times more simulation steps and
considering the liner behavior of the simulation code, we would have an Exec Cmd
(dark gray) time 10 times longer. The rest of the diagram would be the same.
Thus, the longer task execution time, the less relevant will be the overheads
described above for resource utilization.

We also run \wfcg on 2000 compute nodes (+1 node for a RP sub-agent), doubling
the number of tasks and DVMs compared to the run with 1000 nodes. At that scale,
we observed three main issues: (i) DVM startup failure (1 DVM failed after
startup and 1 DVM did not start); (ii) an internal failure of PRRTE (``the
topology information for the following node is missing''); and (iii) lost
connectivity with the DVMs (``PRUN: DEFHANDLER WITH STATUS
LOST\_CONNECTION\_TO\_SERVER(-101)''). The majority of tasks were successfully
completed (11802 out of 12000), but those issues prevented RP Task Manager to
gracefully handle their termination.

\jhanote{Placeholder for Flux experiments}

\input{platforms-usage}

